Omni6D: Large-Vocabulary 3D Object Dataset for Category-Level 6D Object Pose Estimation

6D object pose estimation aims at determining an object's translation, rotation, and scale, typically from a single RGBD image. Recent advancements have expanded this estimation from instance-level to category-level, allowing models to generalize across unseen instances within the same category. However, this generalization is limited by the narrow range of categories covered by existing datasets, such as NOCS, which also tend to overlook common real-world challenges like occlusion. To tackle these challenges, we introduce Omni6D, a comprehensive RGBD dataset featuring a wide range of categories and varied backgrounds, elevating the task to a more realistic context. 1) The dataset comprises an extensive spectrum of 166 categories, 4688 instances adjusted to the canonical pose, and over 0.8 million captures, significantly broadening the scope for evaluation. 2) We introduce a symmetry-aware metric and conduct systematic benchmarks of existing algorithms on Omni6D, offering a thorough exploration of new challenges and insights. 3) Additionally, we propose an effective fine-tuning approach that adapts models from previous datasets to our extensive vocabulary setting. We believe this initiative will pave the way for new insights and substantial progress in both the industrial and academic fields, pushing forward the boundaries of general 6D pose estimation.

==> sec/abstract.tex <==
\begin{abstract}
6D object pose estimation aims at determining an object's translation, rotation, and scale, typically from a single RGBD image. Recent advancements have expanded this estimation from instance-level to category-level, allowing models to generalize across unseen instances within the same category.
However, this generalization is limited by the narrow range of categories covered by existing datasets, such as NOCS, which also tend to overlook common real-world challenges like occlusion.
To tackle these challenges, we introduce \textbf{Omni6D}, a comprehensive RGBD dataset featuring a wide range of categories and varied backgrounds, elevating the task to a more realistic context. 
\textbf{1)} The dataset comprises an extensive spectrum of \textbf{166} categories, \textbf{4688} instances, and over \textbf{0.8 million} captures, significantly broadening the scope for evaluation.
\textbf{2)} We conducted systematic benchmarks of existing algorithms on Omni6D, offering a thorough exploration of new challenges and insights. 
\textbf{3)} Additionally, we propose an effective fine-tuning approach that adapts models from previous datasets to our extensive vocabulary setting. Notably, in a 48-category evaluation, this method achieved a maximum of 64.03\% relative improvement in the $5^\circ2~cm$ metric.
We believe this initiative will pave the way for new insights and substantial progress in both the industrial and academic fields, pushing forward the boundaries of general 6D pose estimation. 
% check
  \keywords{6DoF Pose Estimation \and Large Vocabulary Dataset \and Metrics and Benchmarks}
\end{abstract}

==> supply_figures/cluster.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=\linewidth]{supply_figures/cluster.png}
   \caption{\textbf{Clustering results whithin Omni6D dataset.} The angle of each sector in the chart reflects the relative size of the instance count within that category.}
   \label{fig:cluster}
\end{figure}

==> supply_figures/diversity.tex <==
\begin{figure}[t]
  \centering
   \includegraphics[width=1.01\linewidth]{supply_figures/diversity.png}
   \caption{\textbf{Intra-class diversity in Omni6D for various categories.} We measure the diversity of instances within a category using the mean Chamfer distance of all pairwise pairs within that category. Images are sorted in descending order based on the intra-class diversity of each category in Omni6D$_{train}$.}
   \label{fig:diversity}
\end{figure}
